Wide Activation for Efficient and Accurate Image Super-Resolution

In this report we demonstrate that with same parameters and computational budgets, models with wider features before ReLU activation have significantly better performance for single image super-resolution (SISR). The resulted SR residual network has a slim identity mapping pathway with wider (\(2\times\) to \(4\times\)) channels before activation in each residual block. To further widen activation (\(6\times\) to \(9\times\)) without computational overhead, we introduce linear low-rank convolution into SR networks and achieve even better accuracy-efficiency tradeoffs. In addition, compared with batch normalization or no normalization, we find training with weight normalization leads to better accuracy for deep super-resolution networks. Our proposed SR network \textit{WDSR} achieves better results on large-scale DIV2K image super-resolution benchmark in terms of PSNR with same or lower computational complexity. Based on WDSR, our method also won 1st places in NTIRE 2018 Challenge on Single Image Super-Resolution in all three realistic tracks. Experiments and ablation studies support the importance of wide activation for image super-resolution. Code is released at: https://github.com/JiahuiYu/wdsr_ntire2018

==> tabs/div2k_table.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Scale        & SRResNet     & MDSR         & \begin{tabular}[c]{@{}c@{}}EDSR\\ (1.5M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}EDSR\\ (43M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}WDSR\\ (1.2M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}WDSR\\ (37M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}WDSR+\\ (37M)\end{tabular} \\ \hline
\(\times 2\) & 34.44/0.9665 & 34.96/0.9692 & 34.55/0.9671                                          & 35.03/0.9695                                         & 34.72                                                 &                                                      & {\color[HTML]{FF0000} 35.11}                          \\ \hline
\(\times 3\) & 30.85/0.9292 & 31.25/0.9338 & 30.90/0.9298                                          & 31.26/0.9340                                         &                                                       & 31.24                                                &                                                       \\ \hline
\(\times 4\) & 28.92/0.8961 & 29.26/0.9016 & 28.94/0.8963                                          & 29.25/0.9017                                         &                                                       &                                                      &                                                       \\ \hline
\end{tabular}
\caption{My caption}
\label{my-label}
\end{table}
